Submodular Optimization over Sliding Windows

Maximizing submodular functions under cardinality constraints lies at the core of numerous data mining and machine learning applications, including data diversification, data summarization, and coverage problems. In this work, we study this question in the context of data streams, where elements arrive one at a time, and we want to design low-memory and fast update-time algorithms that maintain a good solution. Specifically, we focus on the sliding window model, where we are asked to maintain a solution that considers only the last $W$ items. In this context, we provide the first non-trivial algorithm that maintains a provable approximation of the optimum using space sublinear in the size of the window. In particular we give a $\frac{1}{3} - \epsilon$ approximation algorithm that uses space polylogarithmic in the spread of the values of the elements, $\Phi$, and linear in the solution size $k$ for any constant $\epsilon > 0$ . At the same time, processing each element only requires a polylogarithmic number of evaluations of the function itself. When a better approximation is desired, we show a different algorithm that, at the cost of using more memory, provides a $\frac{1}{2} - \epsilon$ approximation and allows a tunable trade-off between average update time and space. This algorithm matches the best known approximation guarantees for submodular optimization in insertion-only streams, a less general formulation of the problem. We demonstrate the efficacy of the algorithms on a number of real world datasets, showing that their practical performance far exceeds the theoretical bounds. The algorithms preserve high quality solutions in streams with millions of items, while storing a negligible fraction of them.

==> applications.tex <==
\section{Applications}
\label{sect:applications}
Submodular optimization has received a large interest in the literature for its vast versatility (\cite{krause2012submodular} provide numerous application examples). Here we only briefly sketch two instantiations of submodular maximization that have wide applications and for which we show experiments in the next section: maximum set coverage and active set selection.


\paragraph{Maximum set coverage} The maximum set coverage problem is a well known NP-Hard problem. In a maximum set coverage instance one wants to select, from a family of subsets of a ground set, a fixed number of sets with maximum cardinality of the union. More precisely, in the slinding window streaming context we are given in input a sequence of sets $v_1,v_2, \ldots$ such that each set  $v_i$ is a subset of the ground set. At any point in time, we want to maintain a set of at most $k$ sets from the current active window, such that the size of their union is maximized. This problem has numerous applications. For instance, the sets might represent content available in an on line service (e.g. videos, items to purchase, ads, check-ins in a location-based system) each of them associated with a subset of users that is interested in them and we want to select $k$ items to show in the front page to maximize the total number of users interested in at least one of them\footnote{Notice that in practice more nuanced variations of this basic problem can be used, including assigning weights to users and allowing partial coverage of users all of which can be casted as submodular maximization (in general many selection problems showing ``diminishing returns'' phenomena can be casted as submodular maximization). Here we experiment with basic set coverage for simplicity as our main purpose is to evaluate our algorithms with a concrete function.}. In this context the items (i.e. the sets) arrive over time at high rates and recency is a key factor, as the home page should mostly show items that are introduced or that received much interest recently. In other examples, the sets in input might be the subset of topics (or labels, tags, etc.) covered by a given item, and again we are interested in showing a limited number of items so that we cover as many topics of interest as possible. Other applications of maximum cover in insertion-only stream has been discussed for instance in~\cite{saha2009maximum}. In our experiments we show two simple applications of set coverage based on public-available data: maintaining a set of recently active point of interests from Gowalla location-based social network check-ins data covering as many users as possible, and analysis DBLP co-authorship data to extract a set of recent researchers covering as many fields as possible.

\paragraph{Active set selection} 
\label{sect:active-set}
Another application of submodular maximization is in the context of the area of data summarization. In this context we want to extract a representative set of $k$ elements from an arbitrary set of items. This procedure finds numerous applications in explorative data analysis and visualization as well as in speeding up machine learning methods. For instance, in a on line system receiving a high velocity stream of event updates (e.g. possible security alerts, news stories, etc.) we want to keep track of $k$ informative events to be shown for diagnostic and visualization purposes and/or conducting more in depth machine learning analysis.
Clearly, in many contexts we only want to present recent items from the stream, as older events are less relevant. A concrete instantiation of this problem is the problem of active set selection with Informative Vector Machine (more details available in \cite{KDD14}) which consists of selecting a set of $k$ items which maximizes a submodular function defined in terms of an information theory based function on the restricted kernel matrix over the selected items. More precisely let $K_{S,S}$ be the restricted kernel matrix over the items $s_1, \ldots s_{|S|} \in S$ i.e. $K_{S,S}(i,j) = \mathcal{K}(s_i,s_j)$ where $\mathcal{K}(s_i,s_j)$ is the similarity of item $i$ and $j$ according to some symmetric positive definite kernel function $\mathcal{K}$. 
In this paper for consistency with previous work, we use the kernel settings of \cite{KDD14}: the items are points in a Euclidean space and $\mathcal{K}=\exp (-|s_i - s_j|^2_2/h^2)$ where $h$ is set to $0.75$. Then the problem we want to address is finding a set $S$ of at most $k$ points maximizing the log-determinant of the following matrix:
$$f(S) = \frac{1}{2} \log \det (\mathbf{I} +\sigma^{-2} K_{S,S})$$
where $\mathbf{I}$ is the identity matrix of size $|S|$ and $\sigma$ is a regularization parameter that we set to $1$ as in \cite{KDD14}. In this context we experiment with a standard dataset in submodular optimization, the Yahoo! front page datasets, were we maintain a set of representative recent users' visits

